Leveraging Eclipse MOSAIC for Modeling and Analyzing Ride-Hailing Services

Ride-hailing services enjoy a large popularity in the sector of individualized mobility. Due to broad availability, ease of use, and competitive pricing strategies, these services have established themselves throughout the last decades. With the increased popularity, ride-hailing providers aimed to consistently improve the efficiency of their services, leading to the inception of novel research questions. Many of which can be effectively tackled using simulation. In this paper, we present such a simulation-based approach using Eclipse MOSAIC in-hand with a large-scale traffic scenario of Berlin. We analyze real-world logbook data including detailed shifts of drivers and discuss how to integrate them with the simulation scenario. Moreover, we present extensions to MOSAIC required for the modeling of the ride-hailing services, utilizing the powerful Application Simulator. Accordingly, as the primary result of this paper, we managed to extend the Eclipse MOSAIC framework to be able to answer research questions in the domain of ride-hailing and ride-sharing. Additionally, in an initial exemplary study, we analyze the traffic and environmental impacts of different, yet basic, rebalancing strategies, finding non-negligible differences in mileages and pollutant emissions. We, furthermore, applied our findings to the entire ride-hailing fleet in the city of Berlin for one year, showcasing the impacts different rebalancing strategies could have on environment and general traffic. To our knowledge, the consideration of environmental factors on a city-wide scale is a novel contribution of this paper, not addressed in previous research.

==> content/90_biography.tex <==
\newpage

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Schrab_small}}]{Karl Schrab} 
received the B.Sc. and M.Sc. degree in Computer Science from the Technische Universität Berlin (TUB) in 2011 and 2015, respectively. 
Since 2015, he is a researcher at the Daimler Center for Automotive IT Innovation (DCAITI), TUB. 
He is the lead developer and maintainer of Eclipse MOSAIC. 
His current research interests include connected and automated mobility, synthetic data and scenario generation, co-simulation, and traffic modeling.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Schweppenhaeuser_small.png}}]{Moritz Schweppenhäuser}
received the B.Sc. in Computer Engineering and the M.Sc. in Computer Science from the Technische Universität Berlin (TUB) in 2018 and 2022, respectively.
Since 2022, he is working as a researcher at the Fraunhofer Institute FOKUS with a focus on topics of Simulated Vehicle Perception and Traffic State Estimation.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Protzmann_small}}]{Robert Protzmann}
received the Ph.D. degree in Computer Engineering from the Technische Universität Berlin in 2018. 
He leads the Simulation and Validation team in Fraunhofer FOKUS, ASCT. 
His research interests cover the simulation of data-driven and cloud-based applications for sustainable mobility, from safe bicycles over electrified to automated vehicles.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/kay.jpg}}]{Kay Massow}
Kay Massow received the Diploma in computer engineering from the Technische Universität Berlin in 2008. In the past, he has worked for Daimler and Volkswagen of America. He is now team leader at the Fraunhofer Institute FOKUS,ASCT and assists teaching and research at the Daimler Center for Automotive IT Innovations, a joint initiative of the Daimler AG and the Technical University of Berlin. He is currently working in the fields of intelligent transport systems, cooperative driving applications, crowdsourced HD map learning, and automotive big data analytics.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Radusch_small}}]{Ilja Radusch}
received the Ph.D. degree in engineering from the Technische Universität Berlin (TUB), Germany.
He is the Head of the Department Automotive Services and Communication Technologies (ASCT), Fraunhofer Institute FOKUS and leads the Daimler Center for Automotive Information Technology Innovations (DCAITI), TUB. 
He works in V2X communication, field operational testing, sensor and ad-hoc networks, and mobile services. 
He has been responsible of industrial and national and international research projects.
\end{IEEEbiography}




% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/author1.png}}]{First A. Author} received the B.S. and M.S. degrees in aerospace engineering from
% the University of Virginia, Charlottesville, in 2001 and the Ph.D. degree in
% mechanical engineering from Drexel University, Philadelphia, PA, in 2008.

% From 2001 to 2004, he was a Research Assistant with the Princeton Plasma
% Physics Laboratory. Since 2009, he has been an Assistant Professor with the
% Mechanical Engineering Department, Texas A{\&}M University, College Station.
% He is the author of three books, more than 150 articles, and more than 70
% inventions. His research interests include high-pressure and high-density
% nonthermal plasma discharge processes and applications, microscale plasma
% discharges, discharges in liquids, spectroscopic diagnostics, plasma
% propulsion, and innovation plasma applications. He is an Associate Editor of
% the journal \emph{Earth, Moon, Planets}, and holds two patents.

% Dr. Author was a recipient of the International Association of Geomagnetism
% and Aeronomy Young Scientist Award for Excellence in 2008, and the IEEE
% Electromagnetic Compatibility Society Best Symposium Paper Award in 2011.
% \end{IEEEbiography}


% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/author2.png}}]{Second B. Author} (M'76--SM'81--F'87) and all authors may include
% biographies. Biographies are often not included in conference-related
% papers. This author became a Member (M) of IEEE in 1976, a Senior
% Member (SM) in 1981, and a Fellow (F) in 1987. The first paragraph may
% contain a place and/or date of birth (list place, then date). Next,
% the author's educational background is listed. The degrees should be
% listed with type of degree in what field, which institution, city,
% state, and country, and year the degree was earned. The author's major
% field of study should be lower-cased.

% The second paragraph uses the pronoun of the person (he or she) and not the
% author's last name. It lists military and work experience, including summer
% and fellowship jobs. Job titles are capitalized. The current job must have a
% location; previous positions may be listed
% without one. Information concerning previous publications may be included.
% Try not to list more than three books or published articles. The format for
% listing publishers of a book within the biography is: title of book
% (publisher name, year) similar to a reference. Current and previous research
% interests end the paragraph.

% The third paragraph begins with the author's
% title and last name (e.g., Dr.\ Smith, Prof.\ Jones, Mr.\ Kajor, Ms.\ Hunter).
% List any memberships in professional societies other than the IEEE. Finally,
% list any awards and work for IEEE committees and publications. If a
% photograph is provided, it should be of good quality, and
% professional-looking. Following are two examples of an author's biography.
% \end{IEEEbiography}



% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/author3.png}}]{Third C. Author, Jr.} (M'87) received the B.S. degree in mechanical
% engineering from National Chung Cheng University, Chiayi, Taiwan, in 2004
% and the M.S. degree in mechanical engineering from National Tsing Hua
% University, Hsinchu, Taiwan, in 2006. He is currently pursuing the Ph.D.
% degree in mechanical engineering at Texas A{\&}M University, College
% Station, TX, USA.

% From 2008 to 2009, he was a Research Assistant with the Institute of
% Physics, Academia Sinica, Tapei, Taiwan. His research interest includes the
% development of surface processing and biological/medical treatment
% techniques using nonthermal atmospheric pressure plasmas, fundamental study
% of plasma sources, and fabrication of micro- or nanostructured surfaces.

% Mr. Author's awards and honors include the Frew Fellowship (Australian
% Academy of Science), the I. I. Rabi Prize (APS), the European Frequency and
% Time Forum Award, the Carl Zeiss Research Award, the William F. Meggers
% Award and the Adolph Lomb Medal (OSA).
% \end{IEEEbiography}
